A Comprehensive Methodology for Volt-VAR Optimization in Active Smart Grids

This paper considers the problem of Volt-VAR Optimization (VVO) in active smart grids. Active smart grids are equipped with distributed generators, distributed storage systems, and tie-line switches that allow for topological reconfiguration. In this paper, the joint operation of the remotely controllable switches, storage units, under load tap changers, and shunt capacitors is formulated for a day-ahead operation scheme. The proposed VVO problem aims at minimizing the expected active power loss in the system and is formulated as a mixed-integer quadratic program. The stochasticity of the wind power generation is addressed through a first-order Markov chain model. Numerical results on a 33-node, 12.66 kV active smart grid using real data from smart meters and wind turbines are presented and compared for various test cases.

==> symbols.tex <==
\section*{Nomenclature}
\addcontentsline{toc}{section}{Nomenclature}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$V_1,V_2,V_3$}]


%
%\item[$N$] Number of nodes in the test system
%\item[$|v_n|, \theta_n$] Voltage magnitude and phase of node $n$
%%\item[$\theta_n$] Voltage phase of node $n$
%\item[$p_n, p_n^G$] Active power demand and generation of node $n$
%\item[$q_n, q_n^G$] Reactive power demand and generation of node $n$
%%\item[$q_n$] Reactive power demand at node $n$
%%\item[$q_n^G$] Reactive power generation at node $n$
%\item[$s_n, s_n^G$] Complex power demand and generation of node $n$
%\item[$p_{mn}, q_{mn}$] Active and reactive power flowing from node $m$ to node $n$
%\item[$s_{mn}$] Complex power flowing from node $m$ to node $n$
%\item[$\mathcal{L}$] Set of all lines that connect the nodes of the system together in a configuration
%\item[$\mathcal{N}^\mathcal{L}_n$] Set of all nodes connected to node $n$ via a line in $\mathcal{L}$
%\item[$\mathcal{S}_\text{sub}$] Set of substation nodes
%\item[$z_l$] Impedance of line $l$
%\item[$r_l, x_l$] Resistance and reactance of line $l$
%\item[$\mathbf{b}$] Vector of nominal storage unit capacities (kWh)
%\item[$\mathbf{c}$] Vector of rated reactive power generation of capacitors (kvar)
%\item[$\omega$] Relative cost of capacities to storage units
%\item[$p^\text{DSS}_n(d,h)$] Active power absorbed (during peak hours) and injected (during off-peak hours)
%by storage unit installed at node $n$ and on day $d$ and hour $h$
%\item[$\mathcal{H}_p$ and $\mathcal{H}_o$] Set of peak and off-peak hours
%\item[$q^G_n(d,h)$] Reactive power injected to the grid during peak hours
%by capacitor installed at node $n$ and on day $d$ and hour $h$
%\item[$\mathbf{p}^{\text{DSS},max}$] Vector of maximum rated power of the storage units that can be installed on the nodes
%\item[$\gamma_{\text{DOD}}$] Depth of Discharge (DOD) of the storage units
%\item[$\beta_{ch}, \beta_{dis}$] The charging and discharging efficiencies of the storage units
%\item[$\mathbf{b}^{max}$] Vector of maximum amount of storage capacity that can be installed on the nodes
%\item[$\mathbf{c}^{max}$] Vector of maximum amount of capacitor power rating that can be installed on the nodes
%\item[$\mathbf{v}^{min}, \mathbf{v}^{max}$] Vectors of minimum and maximum voltage limits
%\item[$|s^{max}_{nm}|$] Maximum apparent power that can flow in the line between node $n$ and $m$.
%\item[$P^{\text{rev}}_{n}$] Maximum active power that can flow to the substation $n$ in reverse direction
%\item[$b_\text{base}$] Base capacity of storage units
%\item[$c_\text{base}$] Base power rating of capacitors
%\item[$\lambda_\text{DSS}$] Ratio of the capacity to power rating of the storage units
%\item[$\mathcal{L}_\infty$] The configuration of the system when all switches are closed
%\item[$y_{nm}$] Binary variable representing if node $n$ is connected to node $m$
%\item[$k_n$] Fictitious load on node $n$
%\item[$k_{nm}$] Fictitious power flowing from node $n$ towards node $m$


%Scalars
\item[$N$] Number of nodes in the test system
\item[$|v_n|, \theta_n$] Voltage magnitude and phase of node $n$
%\item[$\theta_n$] Voltage phase of node $n$
\item[$p_n, p_n^G$] Active power demand and generation of node $n$
\item[$q_n, q_n^G$] Reactive power demand and generation of node $n$
%\item[$q_n$] Reactive power demand at node $n$
%\item[$q_n^G$] Reactive power generation at node $n$
\item[$s_n, s_n^G$] Complex power demand and generation of node $n$
\item[$p_{mn}, q_{mn}$] Active and reactive power flowing from node $m$ to node $n$
\item[$s_{mn}$] Complex power flowing from node $m$ to node $n$
\item[$z_l$] Impedance of line $l$
\item[$r_l, x_l$] Resistance and reactance of line $l$
\item[$\omega$] Relative cost of capacities to storage units
\item[$p^\text{DSS}_n(d,h)$] Active power absorbed (during peak hours) and injected (during off-peak hours)
by storage unit installed at node $n$ and on day $d$ and hour $h$
\item[$q^G_n(d,h)$] Reactive power injected to the grid during peak hours
by capacitor installed at node $n$ and on day $d$ and hour $h$
\item[$\gamma_{\text{DOD}}$] Depth of Discharge (DOD) of the storage units
\item[$\beta_{ch}, \beta_{dis}$] The charging and discharging efficiencies of the storage units
\item[$|s^{max}_{nm}|$] Maximum apparent power that can flow in the line between node $n$ and $m$.
\item[$P^{\text{rev}}_{n}$] Maximum active power that can flow to the substation $n$ in reverse direction
\item[$b_\text{base}$] Base capacity of storage units
\item[$c_\text{base}$] Base power rating of capacitors
\item[$\lambda_\text{DSS}$] Ratio of the capacity to power rating of the storage units
\item[$y_{nm}$] Binary variable representing if node $n$ is connected to node $m$
\item[$k_n$] Fictitious load on node $n$
\item[$k_{nm}$] Fictitious power flowing from node $n$ towards node $m$

%Sets
\item[$\mathcal{L}$] Set of all lines that connect the nodes of the system together in a configuration
\item[$\mathcal{N}^\mathcal{L}_n$] Set of all nodes connected to node $n$ via a line in $\mathcal{L}$
\item[$\mathcal{S}_\text{sub}$] Set of substation nodes
\item[$\mathcal{H}_p$ and $\mathcal{H}_o$] Set of peak and off-peak hours
\item[$\mathcal{L}_\infty$] The configuration of the system when all switches are closed

%Vectors
\item[$\mathbf{b}$] Vector of nominal storage unit capacities (kWh)
\item[$\mathbf{c}$] Vector of rated reactive power generation of capacitors (kvar)
\item[$\mathbf{p}^{\text{DSS},max}$] Vector of maximum rated power of the storage units that can be installed on the nodes
\item[$\mathbf{b}^{max}$] Vector of maximum amount of storage capacity that can be installed on the nodes
\item[$\mathbf{c}^{max}$] Vector of maximum amount of capacitor power rating that can be installed on the nodes
\item[$\mathbf{v}^{min}, \mathbf{v}^{max}$] Vectors of minimum and maximum voltage limits

\end{IEEEdescription}



